The Convergence of Discrete Uniformizations for Genus Zero Surfaces

The notion of discrete conformality proposed by Luo and Bobenko-Pinkall-Springborn on triangle meshes has rich mathematical theories and wide applications. Gu et al. proved that the discrete uniformizations approximate the continuous uniformization for closed surfaces of genus $\geq 1$, given that the approximating triangle meshes are reasonably good. In this paper, we generalize this result to the remaining case of genus-zero surfaces, by reducing it to planar cases via stereographic projections.

==> sreference.tex <==
@article{bucking2018c,
  title={$C^{\infty}$-Convergence of Conformal Mappings for Conformally Equivalent Triangular Lattices},
  author={B{\"u}cking, Ulrike},
  journal={Results in Mathematics},
  volume={73},
  number={2},
  pages={1--21},
  year={2018},
  publisher={Springer}
}

@article{luo2020discrete,
  title={Discrete conformal geometry of polyhedral surfaces and its convergence},
  author={Luo, Feng and Sun, Jian and Wu, Tianqi},
  journal={arXiv preprint arXiv:2009.12706},
  year={2020}
}

@article{rivin1994intrinsic,
  title={Intrinsic geometry of convex ideal polyhedra in hyperbolic 3-space},
  author={Rivin, Igor},
  journal={Lecture Notes in Pure and Applied Mathematics},
  pages={275--291},
  year={1994},
  publisher={MARCEL DEKKER AG}
}

@article{springborn2008conformal,
  title={Conformal Equivalence of Triangle Meshes},
  author={Springborn, Boris and Schr{\"o}der, Peter and Pinkall, Ulrich},
  journal={ACM Transactions on Graphics},
  volume={27},
  number={3},
  pages={Art--No},
  year={2008},
  publisher={Association for Computing Machinery}
}

@misc{wu2020convergence,
	title={The Convergence of Discrete Uniformizations for Closed Surfaces}, 
	author={Tianqi Wu and Xiaoping Zhu},
	year={2020},
	eprint={2008.06744},
	archivePrefix={arXiv},
	primaryClass={math.GT}
}
@article{alexander1993geometric,
  title={Geometric curvature bounds in Riemannian manifolds with boundary},
  author={Alexander, Stephanie B and Berg, I David and Bishop, Richard L},
  journal={Transactions of the American Mathematical Society},
  volume={339},
  number={2},
  pages={703--716},
  year={1993}
}

@book{petersen2006riemannian,
  title={Riemannian geometry},
  author={Petersen, Peter},
  volume={171},
  year={2006},
  publisher={Springer}

}

@article{2019upper,
  title={Upper curvature bounds and CAT(K)},
  journal={https://lamington.wordpress.com/2012/10/17/upper-curvature-bounds-and-catk/},
}

@article{bridson1999metric,
  title={Metric spaces of non-positive curvature},
  author={Bridson, Martin R and Haefliger, Andr{\'e}},
  year={1999},
  publisher={Springer}
}

@article{dai2018rigidity,
  title={Rigidity of the hexagonal Delaunay triangulated plane},
  author={Dai, Song and Ge, Huabin and Ma, Shiguang},
  journal={arXiv preprint arXiv:1809.05882},
  year={2018}
}

@article{aigerman2015orbifold,
  title={Orbifold Tutte embeddings.},
  author={Aigerman, Noam and Lipman, Yaron},
  journal={ACM Trans. Graph.},
  volume={34},
  number={6},
  pages={190--1},
  year={2015}
}

@article{dym2019linear,
  title={Linear variational principle for Riemann mappings and discrete conformality},
  author={Dym, Nadav and Slutsky, Raz and Lipman, Yaron},
  journal={Proceedings of the National Academy of Sciences},
  volume={116},
  number={3},
  pages={732--737},
  year={2019},
  publisher={National Acad Sciences}
}

@article{luo2011rigidity,
  title={Rigidity of polyhedral surfaces, III},
  author={Luo, Feng},
  journal={Geometry \& Topology},
  volume={15},
  number={4},
  pages={2299--2319},
  year={2011},
  publisher={Mathematical Sciences Publishers}
}

@article{bucking2008approximation,
  title={Approximation of conformal mappings by circle patterns},
  author={B{\"u}cking, Ulrike},
  journal={Geometriae Dedicata},
  volume={137},
  number={1},
  pages={163--197},
  year={2008},
  publisher={Springer}
}



@article{de1990triangulations,
  title={Triangulations presque {\'e}quilat{\'e}rales des surfaces},
  author={De Verdiere, Y Colin and Marin, A and others},
  journal={Journal of Differential Geometry},
  volume={32},
  number={1},
  pages={199--207},
  year={1990},
  publisher={Citeseer}
}

@book{devadoss2011discrete,
  title={Discrete and computational geometry},
  author={Devadoss, Satyan L and O'Rourke, Joseph},
  year={2011},
  publisher={Princeton University Press}
}


@article{matthes2005convergence,
  title={Convergence in discrete Cauchy problems and applications to circle patterns},
  author={Matthes, Daniel},
  journal={Conformal Geometry and Dynamics of the American Mathematical Society},
  volume={9},
  number={1},
  pages={1--23},
  year={2005}
}

@article{lan2007c,
  title={The $C^\infty$-convergence of SG circle patterns to the Riemann mapping},
  author={Lan, Shi-Yi and Dai, Dao-Qing},
  journal={Journal of mathematical analysis and applications},
  volume={332},
  number={2},
  pages={1351--1364},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{schramm1997circle,
  title={Circle patterns with the combinatorics of the square grid},
  author={Schramm, Oded},
  booktitle={Duke Math. J},
  year={1997},
  organization={Citeseer}
}

@article{pinkall1993computing,
  title={Computing discrete minimal surfaces and their conjugates},
  author={Pinkall, Ulrich and Polthier, Konrad},
  journal={Experimental mathematics},
  volume={2},
  number={1},
  pages={15--36},
  year={1993},
  publisher={Taylor \& Francis}
}


@article{springborn2019ideal,
  title={Ideal Hyperbolic Polyhedra and Discrete Uniformization},
  author={Springborn, Boris},
  journal={Discrete \& Computational Geometry},
  pages={1--46},
  year={2019},
  publisher={Springer}
}


@article{hurdal2009discrete,
  title={Discrete conformal methods for cortical brain flattening},
  author={Hurdal, Monica K and Stephenson, Ken},
  journal={Neuroimage},
  volume={45},
  number={1},
  pages={S86--S98},
  year={2009},
  publisher={Elsevier}
}

@article{he1996convergence,
  title={On the convergence of circle packings to the Riemann map},
  author={He, Zheng-Xu and Schramm, Oded},
  journal={Inventiones mathematicae},
  volume={125},
  number={2},
  pages={285--305},
  year={1996},
  publisher={Springer}
}

@article{maskit1999new,
  title={New parameters for Fuchsian groups of genus 2},
  author={Maskit, Bernard},
  journal={Proceedings of the American Mathematical Society},
  volume={127},
  number={12},
  pages={3643--3652},
  year={1999}
}

@article{maskit2001matrices,
  title={Matrices for Fenchel-Nielsen coordinates},
  author={Maskit, Bernard},
  journal={RECON no. 20010088230.; Annales Academiae Scientiarum Fennicae: Mathmatica},
  volume={26},
  number={2},
  pages={267--304},
  year={2001}
}

@book{eells1995two,
  title={Two reports on harmonic maps},
  author={Eells, James and Lemaire, Luc},
  year={1995},
  publisher={World Scientific}
}

@article{schoen1979existence,
  title={Existence of incompressible minimal surfaces and the topology of three dimensional manifolds with non-negative scalar curvature},
  author={Schoen, Richard and Yau, Shing-Tung},
  journal={Annals of Mathematics},
  volume={110},
  number={1},
  pages={127--142},
  year={1979},
  publisher={JSTOR}
}

@article{kajigaya2019uniformizing,
  title={Uniformizing surfaces via discrete harmonic maps},
  author={Kajigaya, Toru and Tanaka, Ryokichi},
  journal={arXiv preprint arXiv:1905.05427},
  year={2019}
}



@article{tewari2006meshing,
  title={Meshing genus-1 point clouds using discrete one-forms},
  author={Tewari, Geetika and Gotsman, Craig and Gortler, Steven J},
  journal={Computers \& Graphics},
  volume={30},
  number={6},
  pages={917--926},
  year={2006},
  publisher={Elsevier}
}

@article{liang2013solving,
  title={Solving partial differential equations on point clouds},
  author={Liang, Jian and Zhao, Hongkai},
  journal={SIAM Journal on Scientific Computing},
  volume={35},
  number={3},
  pages={A1461--A1486},
  year={2013},
  publisher={SIAM}
}

@article{li2009meshless,
  title={Meshless harmonic volumetric mapping using fundamental solution methods},
  author={Li, Xin and Guo, Xiaohu and Wang, Hongyu and He, Ying and Gu, Xianfeng and Qin, Hong},
  journal={IEEE Transactions on Automation Science and Engineering},
  volume={6},
  number={3},
  pages={409--422},
  year={2009},
  publisher={IEEE}
}

@inproceedings{xu2011dynamic,
  title={Dynamic harmonic texture mapping using methods of fundamental solutions},
  author={Xu, Huanhuan and Li, Xin},
  booktitle={2011 6th International Conference on Computer Science \& Education (ICCSE)},
  pages={871--875},
  year={2011},
  organization={IEEE}
}

@article{meng2015theory,
  title={The theory of computational quasi-conformal geometry on point clouds},
  author={Meng, Ting Wei and Lui, Lok Ming},
  journal={arXiv preprint arXiv:1510.05104},
  year={2015}
}

@article{guo2006meshless,
  title={Meshless thin-shell simulation based on global conformal parameterization},
  author={Guo, Xiaohu and Li, Xin and Bao, Yunfan and Gu, Xianfeng and Qin, Hong},
  journal={IEEE transactions on visualization and computer graphics},
  volume={12},
  number={3},
  pages={375--385},
  year={2006},
  publisher={IEEE}
}

@article{wang2008high,
  title={High resolution tracking of non-rigid motion of densely sampled 3D data using harmonic maps},
  author={Wang, Yang and Gupta, Mohit and Zhang, Song and Wang, Sen and Gu, Xianfeng and Samaras, Dimitris and Huang, Peisen},
  journal={International Journal of Computer Vision},
  volume={76},
  number={3},
  pages={283--300},
  year={2008},
  publisher={Springer}
}

@article{gu2018discrete,
  title={A discrete uniformization theorem for polyhedral surfaces},
  author={Gu, Xianfeng David and Luo, Feng and Sun, Jian and Wu, Tianqi and others},
  journal={Journal of differential geometry},
  volume={109},
  number={2},
  pages={223--256},
  year={2018},
  publisher={Lehigh University}
}



@article{hass2015simplicial,
  title={Simplicial energy and simplicial harmonic maps},
  author={Hass, Joel and Scott, Peter},
  journal={Asian Journal of Mathematics},
  volume={19},
  number={4},
  pages={593--636},
  year={2015},
  publisher={International Press of Boston}
}





@article{fuglede2008homotopy,
  title={Homotopy problems for harmonic maps to spaces of nonpositive curvature},
  author={Fuglede, Bent},
  journal={Communications in Analysis and Geometry},
  volume={16},
  number={4},
  pages={681--733},
  year={2008},
  publisher={International Press of Boston}
}

@book{eells2001harmonic,
  title={Harmonic maps between Riemannian polyhedra},
  author={Eells, James and Fuglede, Bent},
  volume={142},
  year={2001},
  publisher={Cambridge university press}
}

@article{izeki2005combinatorial,
  title={Combinatorial harmonic maps and discrete-group actions on Hadamard spaces},
  author={Izeki, Hiroyasu and Nayatani, Shin},
  journal={Geometriae Dedicata},
  volume={114},
  number={1},
  pages={147--188},
  year={2005},
  publisher={Springer}
}

@article{wang2000generalized,
  title={Generalized harmonic maps and representations of discrete groups},
  author={Wang, Mu-Tao},
  journal={Communications in analysis and geometry},
  volume={8},
  number={3},
  pages={545--563},
  year={2000},
  publisher={International Press of Boston}
}

@article{jost2007harmonic,
  title={Harmonic nets in metric spaces},
  author={Jost, J{\"u}rgen and Todjihounde, Leonard},
  journal={Pacific Journal of Mathematics},
  volume={231},
  number={2},
  pages={437--444},
  year={2007},
  publisher={Mathematical Sciences Publishers}
}

@article{korevaar1993sobolev,
  title={Sobolev spaces and harmonic maps for metric space targets},
  author={Korevaar, Nicholas J and Schoen, Richard M},
  journal={Communications in Analysis and Geometry},
  volume={1},
  number={4},
  pages={561--659},
  year={1993},
  publisher={International Press of Boston}
}

@article{de1991comment,
  title={Comment rendre g{\'e}od{\'e}sique une triangulation d’une surface?},
  author={de Verdi\`ere, Y Colin},
  journal={L’Enseignement Math{\'e}matique},
  volume={37},
  pages={201--212},
  year={1991}
}


@incollection{li2001moving,
  title={Moving mesh finite element methods based on harmonic maps},
  author={Li, Ruo and Liu, Wenbin and Tang, Tao and Zhang, Pingwen},
  booktitle={Scientific computing and applications},
  pages={143--156},
  year={2001}
}

@article{joshi2007surface,
  title={Surface-constrained volumetric brain registration using harmonic mappings},
  author={Joshi, Anand A and Shattuck, David W and Thompson, Paul M and Leahy, Richard M},
  journal={IEEE transactions on medical imaging},
  volume={26},
  number={12},
  pages={1657--1669},
  year={2007},
  publisher={IEEE}
}

@article{li2009surface,
  title={Surface mapping using consistent pants decomposition},
  author={Li, Xin and Gu, Xianfeng and Qin, Hong},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={15},
  number={4},
  pages={558--571},
  year={2009},
  publisher={IEEE}
}

@article{wu2015rigidity,
  title={Rigidity of infinite hexagonal triangulation of the plane},
  author={Wu, Tianqi and Gu, Xianfeng and Sun, Jian},
  journal={Transactions of the American Mathematical Society},
  volume={367},
  number={9},
  pages={6539--6555},
  year={2015}
}

@article{crane2013robust,
  title={Robust fairing via conformal curvature flow},
  author={Crane, Keenan and Pinkall, Ulrich and Schr{\"o}der, Peter},
  journal={ACM Transactions on Graphics (TOG)},
  volume={32},
  number={4},
  pages={1--10},
  year={2013},
  publisher={ACM New York, NY, USA}
}

@inproceedings{kittler2018conformal,
  title={Conformal mapping of a 3D face representation onto a 2D image for CNN based face recognition},
  author={Kittler, Josef and Koppen, Paul and Kopp, Philipp and Huber, Patrik and R{\"a}tsch, Matthias},
  booktitle={2018 International Conference on Biometrics (ICB)},
  pages={124--131},
  year={2018},
  organization={IEEE}
}

@article{ben2018multi,
  title={Multi-chart generative surface modeling},
  author={Ben-Hamu, Heli and Maron, Haggai and Kezurer, Itay and Avineri, Gal and Lipman, Yaron},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={6},
  pages={1--15},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{maron2017convolutional,
  title={Convolutional neural networks on surfaces via seamless toric covers.},
  author={Maron, Haggai and Galun, Meirav and Aigerman, Noam and Trope, Miri and Dym, Nadav and Yumer, Ersin and Kim, Vladimir G and Lipman, Yaron},
  journal={ACM Trans. Graph.},
  volume={36},
  number={4},
  pages={71--1},
  year={2017}
}

@article{soliman2018optimal,
  title={Optimal cone singularities for conformal flattening},
  author={Soliman, Yousuf and Slep{\v{c}}ev, Dejan and Crane, Keenan},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={4},
  pages={1--17},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{kim2011blended,
  title={Blended intrinsic maps},
  author={Kim, Vladimir G and Lipman, Yaron and Funkhouser, Thomas},
  journal={ACM transactions on graphics (TOG)},
  volume={30},
  number={4},
  pages={1--12},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@article{lipman2009mobius,
  title={M{\"o}bius voting for surface correspondence},
  author={Lipman, Yaron and Funkhouser, Thomas},
  journal={ACM Transactions on Graphics (TOG)},
  volume={28},
  number={3},
  pages={1--12},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{lui2010optimized,
  title={Optimized conformal surface registration with shape-based landmark matching},
  author={Lui, Lok Ming and Thiruvenkadam, Sheshadri and Wang, Yalin and Thompson, Paul M and Chan, Tony F},
  journal={SIAM Journal on Imaging Sciences},
  volume={3},
  number={1},
  pages={52--78},
  year={2010},
  publisher={SIAM}
}

@inproceedings{hong2006conformal,
  title={Conformal virtual colon flattening},
  author={Hong, Wei and Gu, Xianfeng and Qiu, Feng and Jin, Miao and Kaufman, Arie},
  booktitle={Proceedings of the 2006 ACM symposium on Solid and physical modeling},
  pages={85--93},
  year={2006}
}

@article{boyer2011algorithms,
  title={Algorithms to automatically quantify the geometric similarity of anatomical surfaces},
  author={Boyer, Doug M and Lipman, Yaron and Clair, Elizabeth St and Puente, Jesus and Patel, Biren A and Funkhouser, Thomas and Jernvall, Jukka and Daubechies, Ingrid},
  journal={Proceedings of the National Academy of Sciences},
  volume={108},
  number={45},
  pages={18221--18226},
  year={2011},
  publisher={National Acad Sciences}
}

@article{gu2004genus,
  title={Genus zero surface conformal mapping and its application to brain surface mapping},
  author={Gu, Xianfeng and Wang, Yalin and Chan, Tony F and Thompson, Paul M and Yau, Shing-Tung},
  journal={IEEE transactions on medical imaging},
  volume={23},
  number={8},
  pages={949--958},
  year={2004},
  publisher={IEEE}
}

@article{koehl2013automatic,
  title={Automatic alignment of genus-zero surfaces},
  author={Koehl, Patrice and Hass, Joel},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={36},
  number={3},
  pages={466--478},
  year={2013},
  publisher={IEEE}
}

@article{kharevych2006discrete,
  title={Discrete conformal mappings via circle patterns},
  author={Kharevych, Liliya and Springborn, Boris and Schr{\"o}der, Peter},
  journal={ACM Transactions on Graphics (TOG)},
  volume={25},
  number={2},
  pages={412--438},
  year={2006},
  publisher={ACM New York, NY, USA}
}

@article{dym2019linear,
  title={Linear variational principle for Riemann mappings and discrete conformality},
  author={Dym, Nadav and Slutsky, Raz and Lipman, Yaron},
  journal={Proceedings of the National Academy of Sciences},
  volume={116},
  number={3},
  pages={732--737},
  year={2019},
  publisher={National Acad Sciences}
}

@article{yueh2017efficient,
  title={An efficient energy minimization for conformal parameterizations},
  author={Yueh, Mei-Heng and Lin, Wen-Wei and Wu, Chin-Tien and Yau, Shing-Tung},
  journal={Journal of Scientific Computing},
  volume={73},
  number={1},
  pages={203--227},
  year={2017},
  publisher={Springer}
}

@inproceedings{desbrun2002intrinsic,
  title={Intrinsic parameterizations of surface meshes},
  author={Desbrun, Mathieu and Meyer, Mark and Alliez, Pierre},
  booktitle={Computer graphics forum},
  volume={21},
  number={3},
  pages={209--218},
  year={2002},
  organization={Wiley Online Library}
}

@article{levy2002least,
  title={Least squares conformal maps for automatic texture atlas generation},
  author={L{\'e}vy, Bruno and Petitjean, Sylvain and Ray, Nicolas and Maillot, J{\'e}rome},
  journal={ACM transactions on graphics (TOG)},
  volume={21},
  number={3},
  pages={362--371},
  year={2002},
  publisher={ACM New York, NY, USA}
}


@inproceedings{trefethen1998schwarz,
  title={Schwarz-Christoffel mapping in the computer era},
  author={Trefethen, Lloyd N and Driscoll, Tobin A},
  booktitle={Proceedings of the International Congress of Mathematicians},
  volume={3},
  pages={533--542},
  year={1998},
  organization={Citeseer}
}

@book{stephenson2005introduction,
  title={Introduction to circle packing: The theory of discrete analytic functions},
  author={Stephenson, Kenneth},
  year={2005},
  publisher={Cambridge University Press}
}

@article{driscoll1998numerical,
  title={Numerical conformal mapping using cross-ratios and Delaunay triangulation},
  author={Driscoll, Tobin A and Vavasis, Stephen A},
  journal={SIAM Journal on Scientific Computing},
  volume={19},
  number={6},
  pages={1783--1803},
  year={1998},
  publisher={SIAM}
}

@article{bishop2010conformal,
  title={Conformal mapping in linear time},
  author={Bishop, Christopher J},
  journal={Discrete \& Computational Geometry},
  volume={44},
  number={2},
  pages={330--428},
  year={2010},
  publisher={Springer}
}

@article{kharevych2006discrete,
  title={Discrete conformal mappings via circle patterns},
  author={Kharevych, Liliya and Springborn, Boris and Schr{\"o}der, Peter},
  journal={ACM Transactions on Graphics (TOG)},
  volume={25},
  number={2},
  pages={412--438},
  year={2006},
  publisher={ACM New York, NY, USA}
}

@incollection{bucking2016approximation,
  title={Approximation of conformal mappings using conformally equivalent triangular lattices},
  author={B{\"u}cking, Ulrike},
  booktitle={Advances in Discrete Differential Geometry},
  pages={133--149},
  year={2016},
  publisher={Springer, Berlin, Heidelberg}
}


@article{hurdal2009discrete,
  title={Discrete conformal methods for cortical brain flattening},
  author={Hurdal, Monica K and Stephenson, Ken},
  journal={Neuroimage},
  volume={45},
  number={1},
  pages={S86--S98},
  year={2009},
  publisher={Elsevier}
}


@article{luo2016discrete,
  title={Discrete conformal geometry of polyhedral surfaces and its convergence},
  author={Luo, Feng and Sun, Jian and Wu, Tianqi},
  journal={preprint},
  volume={37},
  year={2020}
}



@article{gu2019convergence,
  title={Convergence of discrete conformal geometry and computation of uniformization maps},
  author={Gu, David and Luo, Feng and Wu, Tianqi},
  journal={Asian Journal of Mathematics},
  volume={23},
  number={1},
  pages={21--34},
  year={2019},
  publisher={International Press of Boston}
}




@article{springborn2017hyperbolic,
  title={Hyperbolic polyhedra and discrete uniformization},
  author={Springborn, Boris},
  journal={arXiv preprint arXiv:1707.06848},
  year={2017}
}


@article{glickenstein2011discrete,
  title={Discrete conformal variations and scalar curvature on piecewise flat two-and three-dimensional manifolds},
  author={Glickenstein, David and others},
  journal={Journal of Differential Geometry},
  volume={87},
  number={2},
  pages={201--238},
  year={2011},
  publisher={Lehigh University}
}

@article{lui2014teichmuller,
  title={Teichmuller mapping (t-map) and its applications to landmark matching registration},
  author={Lui, Lok Ming and Lam, Ka Chun and Yau, Shing-Tung and Gu, Xianfeng},
  journal={SIAM Journal on Imaging Sciences},
  volume={7},
  number={1},
  pages={391--426},
  year={2014},
  publisher={SIAM}
}

@article{lipman2012bounded,
  title={Bounded distortion mapping spaces for triangular meshes},
  author={Lipman, Yaron},
  journal={ACM Transactions on Graphics (TOG)},
  volume={31},
  number={4},
  pages={1--13},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@article{levy2002least,
  title={Least squares conformal maps for automatic texture atlas generation},
  author={L{\'e}vy, Bruno and Petitjean, Sylvain and Ray, Nicolas and Maillot, J{\'e}rome},
  journal={ACM transactions on graphics (TOG)},
  volume={21},
  number={3},
  pages={362--371},
  year={2002},
  publisher={ACM New York, NY, USA}
}

@article{gu2002computing,
  title={Computing conformal structures of surfaces},
  author={Gu, Xianfeng and Yau, Shing-Tung},
  journal={Communications in Information and Systems},
  volume={2},
  number={2},
  pages={121--146},
  year={2002},
  publisher={International Press of Boston}
}



@article{glickenstein2005maximum,
  title={A maximum principle for combinatorial Yamabe flow},
  author={Glickenstein, David},
  journal={Topology},
  volume={44},
  number={4},
  pages={809--825},
  year={2005},
  publisher={Elsevier}
}

@article{glickenstein2005combinatorial,
  title={A combinatorial Yamabe flow in three dimensions},
  author={Glickenstein, David},
  journal={Topology},
  volume={44},
  number={4},
  pages={791--808},
  year={2005},
  publisher={Elsevier}
}

@article{sun2015discrete,
  title={Discrete conformal deformation: algorithm and experiments},
  author={Sun, Jian and Wu, Tianqi and Gu, Xianfeng and Luo, Feng},
  journal={SIAM Journal on Imaging Sciences},
  volume={8},
  number={3},
  pages={1421--1456},
  year={2015},
  publisher={SIAM}
}

@article{gu2018discrete2,
  title={A discrete uniformization theorem for polyhedral surfaces II},
  author={Gu, Xianfeng and Guo, Ren and Luo, Feng and Sun, Jian and Wu, Tianqi and others},
  journal={Journal of differential geometry},
  volume={109},
  number={3},
  pages={431--466},
  year={2018},
  publisher={Lehigh University}
}

@article{gu2018discrete,
  title={A discrete uniformization theorem for polyhedral surfaces},
  author={Gu, Xianfeng David and Luo, Feng and Sun, Jian and Wu, Tianqi and others},
  journal={Journal of differential geometry},
  volume={109},
  number={2},
  pages={223--256},
  year={2018},
  publisher={Lehigh University}
}

@article{bobenko2015discrete,
  title={Discrete conformal maps and ideal hyperbolic polyhedra},
  author={Bobenko, Alexander I and Pinkall, Ulrich and Springborn, Boris A},
  journal={Geometry \& Topology},
  volume={19},
  number={4},
  pages={2155--2215},
  year={2015},
  publisher={Mathematical Sciences Publishers}
}

@article{luo2004combinatorial,
  title={Combinatorial Yamabe flow on surfaces},
  author={Luo, Feng},
  journal={Communications in Contemporary Mathematics},
  volume={6},
  number={05},
  pages={765--780},
  year={2004},
  publisher={World Scientific}
}

@article{rovcek1984quantization,
  title={The quantization of Regge calculus},
  author={Ro{\v{c}}ek, M and Williams, Ruth M},
  journal={Zeitschrift f{\"u}r Physik C Particles and Fields},
  volume={21},
  number={4},
  pages={371--381},
  year={1984},
  publisher={Springer}
}

@article{guo2011local,
  title={Local rigidity of inversive distance circle packing},
  author={Guo, Ren},
  journal={Transactions of the American Mathematical Society},
  volume={363},
  number={9},
  pages={4757--4776},
  year={2011}
}

@incollection{bowers2003planar,
  title={Planar conformal mappings of piecewise flat surfaces},
  author={Bowers, Philip L and Hurdal, Monica K},
  booktitle={Visualization and mathematics III},
  pages={3--34},
  year={2003},
  publisher={Springer}
}

@book{bowers2004uniformizing,
  title={Uniformizing Dessins and BelyiMaps via Circle Packing},
  author={Bowers, Philip L and Stephenson, Kenneth},
  volume={170},
  number={805},
  year={2004},
  publisher={American Mathematical Soc.}
}

@article{chow2003combinatorial,
  title={Combinatorial Ricci flows on surfaces},
  author={Chow, Bennett and Luo, Feng and others},
  journal={Journal of Differential Geometry},
  volume={63},
  number={1},
  pages={97--129},
  year={2003},
  publisher={Lehigh University}
}

@article{de1991principe,
  title={Un principe variationnel pour les empilements de cercles},
  author={De Verdi\`ere, Yves Colin},
  journal={Inventiones mathematicae},
  volume={104},
  number={1},
  pages={655--669},
  year={1991},
  publisher={Springer}
}

@article{he1998thec,
  title={The $C^\infty$-convergence of hexagonal disk packings to the riemann map},
  author={He, Zheng-Xu and Schramm, Oded},
  journal={Acta mathematica},
  volume={180},
  number={2},
  pages={219--245},
  year={1998},
  publisher={Springer}
}

@article{rodin1987convergence,
  title={The convergence of circle packings to the Riemann mapping},
  author={Rodin, Burt and Sullivan, Dennis},
  journal={Journal of Differential Geometry},
  volume={26},
  number={2},
  pages={349--360},
  year={1987},
  publisher={Lehigh University}
}

@article{stephenson2003circle,
  title={Circle packing: a mathematical tale},
  author={Stephenson, Kenneth},
  journal={Notices of the AMS},
  volume={50},
  number={11},
  pages={1376--1388},
  year={2003}
}


@article{sun2015discrete,
  title={Discrete conformal deformation: algorithm and experiments},
  author={Sun, Jian and Wu, Tianqi and Gu, Xianfeng and Luo, Feng},
  journal={SIAM Journal on Imaging Sciences},
  volume={8},
  number={3},
  pages={1421--1456},
  year={2015},
  publisher={SIAM}
}



@inproceedings{gu2003global,
  title={Global conformal surface parameterization},
  author={Gu, Xianfeng and Yau, Shing-Tung},
  booktitle={Proceedings of the 2003 Eurographics/ACM SIGGRAPH symposium on Geometry processing},
  pages={127--137},
  year={2003}
}


@article{gu2002computing,
  title={Computing conformal structure of surfaces},
  author={Gu, Xianfeng and Yau, Shing-Tung},
  journal={arXiv preprint cs/0212043},
  year={2002}
}

@article{gaster2018computing,
  title={Computing discrete equivariant harmonic maps},
  author={Gaster, Jonah and Loustau, Brice and Monsaingeon, L{\'e}onard},
  journal={arXiv preprint arXiv:1810.11932},
  year={2018}
}

@article{gaster2019computing,
  title={Computing harmonic maps between Riemannian manifolds},
  author={Gaster, Jonah and Loustau, Brice and Monsaingeon, L{\'e}onard},
  journal={arXiv preprint arXiv:1910.08176},
  year={2019}
}


@article{choi2016spherical,
  title={Spherical conformal parameterization of genus-0 point clouds for meshing},
  author={Choi, Gary Pui-Tung and Ho, Kin Tat and Lui, Lok Ming},
  journal={SIAM Journal on Imaging Sciences},
  volume={9},
  number={4},
  pages={1582--1618},
  year={2016},
  publisher={SIAM}
}

@article{meng2016tempo,
  title={Tempo: Feature-endowed teichmuller extremal mappings of point clouds},
  author={Meng, Ting Wei and Choi, Gary Pui-Tung and Lui, Lok Ming},
  journal={SIAM Journal on Imaging Sciences},
  volume={9},
  number={4},
  pages={1922--1962},
  year={2016},
  publisher={SIAM}
}

@inproceedings{liang2012geometric,
  title={Geometric understanding of point clouds using Laplace-Beltrami operator},
  author={Liang, Jian and Lai, Rongjie and Wong, Tsz Wai and Zhao, Hongkai},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={214--221},
  year={2012},
  organization={IEEE}
}

@inproceedings{zwicker2004meshing,
  title={Meshing Point Clouds Using Spherical Parameterization.},
  author={Zwicker, Matthias and Gotsman, Craig},
  booktitle={SPBG},
  pages={173--180},
  year={2004}
}


@article{lai2013local,
  title={A local mesh method for solving PDEs on point clouds},
  author={Lai, Rongjie and Liang, Jiang and Zhao, Hong-Kai},
  journal={Inverse Problems \& Imaging},
  volume={7},
  number={3},
  pages={737},
  year={2013},
  publisher={American Institute of Mathematical Sciences}
}

@article{li2014point,
  title={Point integral method for solving poisson-type equations on manifolds from point clouds with convergence guarantees},
  author={Li, Zhen and Shi, Zuoqiang and Sun, Jian},
  journal={arXiv preprint arXiv:1409.2623},
  year={2014}
}

@article{li2017compute,
  title={Compute Quasi-Conformal Map on Point Cloud by Point Integral Method},
  author={Li, Zhen and Shi, Zuoqiang and Sun, Jian},
  year={2017}
}

@inproceedings{belkin2009constructing,
  title={Constructing Laplace operator from point clouds in ℝ d},
  author={Belkin, Mikhail and Sun, Jian and Wang, Yusu},
  booktitle={Proceedings of the twentieth annual ACM-SIAM symposium on Discrete algorithms},
  pages={1031--1040},
  year={2009},
  organization={SIAM}
}


@book{chung1997spectral,
  title={Spectral graph theory},
  author={Chung, Fan R.K.},
  number={92},
  year={1997},
  publisher={American Mathematical Soc.}
}


@article{osserman1978isoperimetric,
  title={The isoperimetric inequality},
  author={Osserman, Robert and others},
  journal={Bulletin of the American Mathematical Society},
  volume={84},
  number={6},
  pages={1182--1238},
  year={1978},
  publisher={American Mathematical Society}
}

@article{gray2006modern,
  title={Modern differential geometry of curves and surfaces with Mathematica},
  author={Gray, Alfred and Abbena, Elsa and Salamon, S and others},
  year={2006},
  publisher={CRC press}
}

@article{mednykh2012brahmagupta,
  title={BRAHMAGUPTA FORMULA FOR CYCLIC QUADRILATERALS IN THE HYPERBOLIC PLANE.},
  author={MEDNYKH, AD},
  journal={Sibirskie Elektronnye Matematicheskie Izvestiia},
  volume={9},
  year={2012}
}

@book{zwillinger2002crc,
  title={CRC standard mathematical tables and formulae},
  author={Zwillinger, Daniel},
  year={2002},
  publisher={CRC press}
}

@phdthesis{frenkel2018area,
  title={On area and volume in spherical and hyperbolic geometry},
  author={Frenkel, Elena},
  year={2018}
}
@article{colindeverdière1990,
	author = "Colin de Verdière, Y. and Marin, A.",
	doi = "10.4310/jdg/1214445044",
	fjournal = "Journal of Differential Geometry",
	journal = "J. Differential Geom.",
	number = "1",
	pages = "199--207",
	publisher = "Lehigh University",
	title = "Triangulations presque équilatérales des surfaces",
	url = "https://doi.org/10.4310/jdg/1214445044",
	volume = "32",
	year = "1990"
}

